Learning dynamical systems with hit-and-run random feature maps

We show how random feature maps can be used to forecast dynamical systems with excellent forecasting skill. We consider the tanh activation function and judiciously choose the internal weights in a data-driven manner such that the resulting features explore the nonlinear, non-saturated regions of the activation function. We introduce skip connections and construct a deep variant of random feature maps by combining several units. To mitigate the curse of dimensionality, we introduce localization where we learn local maps, employing conditional independence. Our modified random feature maps provide excellent forecasting skill for both single trajectory forecasts as well as long-time estimates of statistical properties, for a range of chaotic dynamical systems with dimensions up to 512. In contrast to other methods such as reservoir computers which require extensive hyperparameter tuning, we effectively need to tune only a single hyperparameter, and are able to achieve state-of-the-art forecast skill with much smaller networks.

==> tikz/DeepSkip.tex <==
% \documentclass{standalone}
% \usepackage{tikz}
% \usetikzlibrary{positioning, calc}
% \usetikzlibrary{arrows.meta}
% \begin{document}

% \tikzset{>={Latex[width=2mm,length=2mm]}}
% \begin{tikzpicture}[node distance=1.5cm]
% \tikzstyle{every node}=[font=\large]
%     % First set of rectangles
%     \begin{scope}[shift={(-3.8,0)}]
%         \node[draw, rectangle, minimum width=0.2cm, minimum height=1.5cm] (x1) {};
%         \node[rectangle, above =0.1cm of x1, xshift=-0cm] (x1t) {$\mathbf{u}_n$};
%         \node[draw, rectangle, minimum width=0.2cm, minimum height=1.5cm, below=of x1] (x2) {};
%         \node[rectangle, above =0.1cm of x2, xshift=-0cm] (x2t) {$\mathbf{u}_n$};
%         \coordinate (midpoint1) at ($(x1.south)!0.5!(x2.north)$);
%         \node[circle, draw, inner sep=0pt, minimum size=0.6cm, right=1cm of midpoint1] (concat1) {$\|$};
%         \node[draw, rectangle, minimum width=2cm, minimum height=2cm, right=1.5cm of concat1] (b1) {SkipRFM};

%         % Add circles to x1
%         \foreach \i in {1,...,3} {
%             \node[circle, draw, fill=blue, inner sep=0pt, minimum size=0.2cm] at ($(x1.north)!{(\i-0.5)/3}!(x1.south)$) {};
%         }

%         % Add circles to x2
%         \foreach \i in {1,...,3} {
%             \node[circle, draw, fill=blue, inner sep=0pt, minimum size=0.2cm] at ($(x2.north)!{(\i-0.5)/3}!(x2.south)$) {};
%         }

%         % Connections to concatenation node
%         \draw[->] (x1.east) -- (concat1.west);
%         \draw[->] (x2.east) -- (concat1.west);
%         \draw[->] (concat1.east) -- (b1.west);
%     \end{scope}

%     % Second set of rectangles
%     \begin{scope}[shift={(4.1cm,0)}]
%         \node[draw, rectangle, minimum width=0.2cm, minimum height=1.5cm] (y1) {};
%         \node[draw, rectangle, minimum width=0.2cm, minimum height=1.5cm, below=of y1] (y2) {};
%         \coordinate (midpoint2) at ($(y1.south)!0.5!(y2.north)$);
%         \node[circle, draw, inner sep=0pt, minimum size=0.6cm, right=1cm of midpoint2] (concat2) {$\|$};
%         \node[draw, rectangle, minimum width=2cm, minimum height=2cm, right=1.5cm of concat2] (b2) {SkipRFM};

%         % Add circles to y1
%         \foreach \i in {1,...,3} {
%             \node[circle, draw, fill=blue, inner sep=0pt, minimum size=0.2cm] at ($(y1.north)!{(\i-0.5)/3}!(y1.south)$) {};
%         }

%         % Add circles to y2
%         \foreach \i in {1,...,3} {
%             \node[circle, draw, fill=orange, inner sep=0pt, minimum size=0.2cm] at ($(y2.north)!{(\i-0.5)/3}!(y2.south)$) {};
%         }

%         % Connections to concatenation node
%         \draw[->] (y1.east) -- (concat2.west);
%         \draw[->] (y2.east) -- (concat2.west);
%         \draw[->] (concat2.east) -- (b2.west);

%         % Arrow from previous big rectangle to current lower rectangle
%         \draw[->] (b1.east) -- ($(y2.west) + (0,0.5)$);
%     \end{scope}

%     % Third set of rectangles
%     \begin{scope}[shift={(12cm,0)}]
%         \node[draw, rectangle, minimum width=0.2cm, minimum height=1.5cm] (z1) {};
%         \node[draw, rectangle, minimum width=0.2cm, minimum height=1.5cm, below=of z1] (z2) {};
%         \coordinate (midpoint3) at ($(z1.south)!0.5!(z2.north)$);
%         \node[circle, draw, inner sep=0pt, minimum size=0.6cm, right=1cm of midpoint3] (concat3) {$\|$};
%         \node[draw, rectangle, minimum width=2cm, minimum height=2cm, right=1.5cm of concat3] (b3) {SkipRFM};

%         % Add circles to z1
%         \foreach \i in {1,...,3} {
%             \node[circle, draw, fill=blue, inner sep=0pt, minimum size=0.2cm] at ($(z1.north)!{(\i-0.5)/3}!(z1.south)$) {};
%         }

%         % Add circles to z2
%         \foreach \i in {1,...,3} {
%             \node[circle, draw, fill=purple, inner sep=0pt, minimum size=0.2cm] at ($(z2.north)!{(\i-0.5)/3}!(z2.south)$) {};
%         }

%         % Connections to concatenation node
%         \draw[->] (z1.east) -- (concat3.west);
%         \draw[->] (z2.east) -- (concat3.west);
%         \draw[->] (concat3.east) -- (b3.west);

%         % Arrow from previous big rectangle to current lower rectangle
%         \draw[->] (b2.east) -- ($(z2.west) + (0,0.5)$);
%     \end{scope}

%     % Fourth bottom rectangle moved to center
%     \begin{scope}[shift={(19.5cm,-1.5cm)}]
%         \node[draw, rectangle, minimum width=0.2cm, minimum height=1.5cm] (w2) {};
%         \node[rectangle, above =0.1cm of w2, xshift=-0.3cm] (w2t) {estimate of $\mathbf{u}_{n+1}$};

%         % Add circles to w2
%         \foreach \i in {1,...,3} {
%             \node[circle, draw, fill=red, inner sep=0pt, minimum size=0.2cm] at ($(w2.north)!{(\i-0.5)/3}!(w2.south)$) {};
%         }

%         % Arrow from previous big rectangle to current lower rectangle
%         \draw[->] (b3.east) -- ($(w2.west) + (0,0)$);
%     \end{scope}

%     % Add skip connections with addition nodes
%     \draw[->] (x2) -- ($(x2.east)!0.5!(y2.west)$);
%     \node[circle, draw, fill=white, inner sep=0pt, minimum size=0.6cm] (add1) at ($(x2.east)!0.5!(y2.west)$) {$+$};
%     \draw[->] (add1) -- (y2.west);

%     \draw[->] (y2) -- ($(y2.east)!0.5!(z2.west)$);
%     \node[circle, draw, fill=white, inner sep=0pt, minimum size=0.6cm] (add2) at ($(y2.east)!0.5!(z2.west)$) {$+$};
%     \draw[->] (add2) -- (z2.west);

%     % L-shaped skip connection for z2 to w2
%     \node[circle, draw, fill=white, inner sep=0pt, minimum size=0.6cm] (add3) at ($(z2.east)+(3.8,0)$) {$+$};
%     \draw[-] (z2.east) -- (add3.west);
%     \draw[->] (add3.east) -- ($(add3.east)+(1.5,0)$) -- ($(w2.west)+(0,0)$);

%     % Top connections with "=" nodes
%     \draw[->] (x1) -- ($(x1.east)!0.5!(y1.west)$);
%     \node[circle, draw, fill=white, inner sep=0pt, minimum size=0.6cm] (eq1) at ($(x1.east)!0.5!(y1.west)$) {$=$};
%     \draw[->] (eq1) -- (y1.west);

%     \draw[->] (y1) -- ($(y1.east)!0.5!(z1.west)$);
%     \node[circle, draw, fill=white, inner sep=0pt, minimum size=0.6cm] (eq2) at ($(y1.east)!0.5!(z1.west)$) {$=$};
%     \draw[->] (eq2) -- (z1.west);

% \end{tikzpicture}
% \end{document}


==> tikz/RFM.tex <==
% \documentclass[A4,12pt,twosided]{article}
% \usepackage{geometry}                % See geometry.pdf to learn the layout options. There are lots.
% \geometry{a4paper}                   % ... or a4paper or a5paper or ... 
% %\geometry{landscape}                % Activate for for rotated page geometry
% %\usepackage[parfill]{parskip}    % Activate to begin paragraphs with an empty line rather than an indent
% \usepackage{url}
% \usepackage{graphicx}
% %\usepackage{algorithm}
% %\usepackage{algorithmic}
% \usepackage[algoruled,boxed,lined,ruled,linesnumbered]{algorithm2e}
% \SetKwInOut{Parameter}{Parameters}
% \SetKwComment{Comment}{/* }{ */}
% %\usepackage{algpseudocode}
% \usepackage{amssymb}
% \usepackage{epstopdf}
% \usepackage{color}
% \usepackage{amsmath}
% \usepackage{amsthm}
% \DeclareGraphicsRule{.tif}{png}{.png}{`convert #1 `dirname #1`/`basename #1 .tif`.png}

% \usepackage{url}
% \usepackage[square,numbers]{natbib}
% \usepackage{subeqnarray}
% \bibliographystyle{abbrvnat}


% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{xcolor}         % colors
% \usepackage{graphicx}

% \usepackage{amsmath}
% %\usepackage{caption}
% \usepackage{subcaption}
% \usepackage{tikz}
% \usepackage{tikz-network}
% \usetikzlibrary{calc}
% \usepackage{tikzpagenodes}
% \usetikzlibrary{shadows,matrix} % Shadows for nodes
% \usepackage{nicematrix}
% \usetikzlibrary{arrows.meta, calc, backgrounds}
% \usepackage[outline]{contour} % glow around text
% \contourlength{1.4pt}


% %% no page numebring
% \usepackage{nopageno} 
 
% % %--------------------------------------------------------------------------
% % %  drawing networks 
% % %--------------------------------------------------------------------------
% \definecolor{cadmiumred}{rgb}{0.89, 0.0, 0.13}
% \definecolor{bleudefrance}{rgb}{0.19, 0.55, 0.91}


% % This is the style settings for nodes
% \tikzset{
%  %    dep/.style={circle,minimum size=#1,fill=orange!20,draw=orange,
% %    dep/.style={circle,minimum size=#1,fill=orange!40,draw=orange,
% %               general shadow={fill=gray!60,shadow xshift=1pt,shadow yshift=-1pt}},
% %    dep/.default=0.25cm,
% %    cli/.style={circle,minimum size=#1,fill=white,draw,
% %                general shadow={fill=gray!40,shadow xshift=1pt,shadow yshift=-1pt}},
% %    cli/.default=0.25cm,
% %    spl/.style={cli=#1,append after command={
% %                  node[circle,draw,dotted,
% %                       minimum size=1.5cm] at (\tikzlastnode.center) {}}},
% %    spl/.default=0.25cm,
% %    dep0/.style={circle,minimum size=#1,fill=bleudefrance!60,draw=bleudefrance,
% %                general shadow={fill=gray!40,shadow xshift=1pt,shadow yshift=-1pt}},
% %    dep0/.default=0.25cm,
% %    dep1/.style={circle,minimum size=#1,fill=cadmiumred!60,draw=cadmiumred,
% %                general shadow={fill=gray!40,shadow xshift=1pt,shadow yshift=-1pt}},
% %    dep1/.default=0.25cm,
% %    c1/.style={-stealth,very thick,red!80!black},
% %    v2/.style={-stealth,very thick,yellow!65!black},
% %    v4/.style={-stealth,very thick,purple!70!black}
% %
% % input nodes 
%     inp/.style={circle, minimum size=3mm, fill=bleudefrance!40, draw=bleudefrance, inner sep=1pt, 
%                       general shadow={fill=gray!40,shadow xshift=1pt,shadow yshift=-1pt}},
%     inp/.default=0.05cm,
% % horizontal nodes 
%      inp_b/.style={circle, minimum size=3mm, fill=bleudefrance!40, draw=black, inner sep=1pt, 
%                           general shadow={fill=gray!40,shadow xshift=1pt,shadow yshift=-1pt}},
%      inp_b/.default=0.05cm,
%      %
%      oup_b/.style={circle, minimum size=3mm, fill=cadmiumred!40, draw=black, inner sep=1pt, 
%                           general shadow={fill=gray!40,shadow xshift=1pt,shadow yshift=-1pt}},
%      oup_b/.default=0.05cm,
%  % hidden nodes 
%     hip/.style={circle, minimum size=3mm, fill=orange!40, draw=orange, inner sep=1pt, 
%                       general shadow={fill=gray!40,shadow xshift=1pt,shadow yshift=-1pt}},
%     hip/.default=0.05cm,
% % output nodes 
%     oup/.style={circle, minimum size=3mm, fill=cadmiumred!40, draw=cadmiumred, inner sep=1pt, 
%                       general shadow={fill=gray!40,shadow xshift=1pt,shadow yshift=-1pt}},
%     oup/.default=0.05cm,
%   }


% % %--------------------------------------------------------------------------
% % %  darwing brackets for vectors/matrices etc 
% % %--------------------------------------------------------------------------
% \tikzset{
%     ncbar angle/.initial=90,
%     ncbar/.style={
%         to path=(\tikztostart)
%         -- ($(\tikztostart)!#1!\pgfkeysvalueof{/tikz/ncbar angle}:(\tikztotarget)$)
%         -- ($(\tikztotarget)!($(\tikztostart)!#1!\pgfkeysvalueof{/tikz/ncbar angle}:(\tikztotarget)$)!\pgfkeysvalueof{/tikz/ncbar angle}:(\tikztostart)$)
%         -- (\tikztotarget)
%     },
%     ncbar/.default=0.5cm,
% }

% \tikzset{square left brace/.style={ncbar=0.25cm}}
% \tikzset{square right brace/.style={ncbar=-0.25cm}}

% \tikzset{round left paren/.style={ncbar=0.5cm,out=120,in=-120}}
% \tikzset{round right paren/.style={ncbar=0.5cm,out=60,in=-60}}



% % %--------------------------------------------------------------------------
% % %  FIGURES
% % %--------------------------------------------------------------------------

% \begin{document}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% % STANDARD RFM
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}[h]
% 	\centering
% \begin{tikzpicture}
% \begin{scope}[local bounding box=graph]

% %% TEXT
%  \node[text width=3cm, align = center] at (-2,-3) {\Large input};
%  \node[text width=3cm, align = center] at (12,-3) {\Large output};
%  \node[text width=5cm, align = center] at (0.75,4) {\Large $\mathbb{R}^{D_r\times D} \ni (W_{\rm{in}},b_{\rm{in}})$};
%  \node[text width=3.5cm, align = center] at (8.35,4) {\Large $W\in \mathbb{R}^{D\times D_r}$};
%  \node[text width=6cm, align = center] at (5,-6.75) {\Large $z_i = \tanh({W_{\rm{in}}}_{i,j} x_j + {b_{\rm{in}}}_i)$};


% %% INPUT NODES
%    \draw [black, thick] (-2.3,-2.4) to [square left brace ] (-2.3,2.4);
%     \node[inp] (i1) at (-2,-2) {$x_D$};
%     \node[inp] (i2) at (-2,0) {$x_j$};
%     \node[inp] (i3) at (-2,2) {$x_1$};
%     \draw[dashed] (i1) to (i2);
%     \draw[dashed] (i2) to (i3);
%     \draw [black, thick] (-1.7,-2.4) to [square right brace ] (-1.7,2.4);

% %% horizontal links
%     \node[inp_b] (i1b) at (1.,-2) {};
%     \node[inp_b] (i2b) at (1.,0) {};
%     \node[inp_b] (i3b) at (1.,2) {};

%      \draw[thick,bleudefrance!40] (i1) -- (i1b);
%      \draw[thick,bleudefrance!40] (i2) -- (i2b);
%      \draw[thick,bleudefrance!40] (i3) -- (i3b);

% %% HIDDEN NODES
%      \filldraw[color=orange!40, fill=orange!40, fill opacity=0.1, rounded corners=1cm](4,-5.75) rectangle (6,5.75);

%     \node[hip] (z1) at (5,-5) {$z_{D_r}$};
%     \node[hip] (z2) at (5,0) {$z_\ell$};
%     \node[hip] (z3) at (5,3) {$z_3$};
%     \node[hip] (z4) at (5,4) {$z_2$};
%     \node[hip] (z5) at (5,5) {$z_1$};
%     \draw[dashed] (z1) to (z2);
%     \draw[dashed] (z2) to (z3);
    
% %% draw lines input --> hidden
%      \draw[opacity=0.6] (i1b) -- (z1);
%      \draw[opacity=0.6] (i1b) -- (z2);
%      \draw[opacity=0.6] (i1b) -- (z3);
%      \draw[opacity=0.6] (i1b) -- (z4);
%      \draw[opacity=0.6] (i1b) -- (z5);
        
%      \draw[opacity=0.6] (i2b) -- (z1);
%      \draw[opacity=0.6] (i2b) -- (z2);
%      \draw[opacity=0.6] (i2b) -- (z3);
%      \draw[opacity=0.6] (i2b) -- (z4);
%      \draw[opacity=0.6] (i2b) -- (z5);

%      \draw[opacity=0.6] (i3b) -- (z1);
%      \draw[opacity=0.6] (i3b) -- (z2);
%      \draw[opacity=0.6] (i3b) -- (z3);
%      \draw[opacity=0.6] (i3b) -- (z4);
%      \draw[opacity=0.6] (i3b) -- (z5);


% %% draw lines hidden --> output 
%     \node[oup_b] (o1b) at (9,-2) {};
%     \node[oup_b] (o2b) at (9,0) {};
%     \node[oup_b] (o3b) at (9,2) {};

%      \draw[opacity=0.6] (o1b) -- (z1);
%      \draw[opacity=0.6] (o1b) -- (z2);
%      \draw[opacity=0.6] (o1b) -- (z3);
%      \draw[opacity=0.6] (o1b) -- (z4);
%      \draw[opacity=0.6] (o1b) -- (z5);
        
%      \draw[opacity=0.6] (o2b) -- (z1);
%      \draw[opacity=0.6] (o2b) -- (z2);
%      \draw[opacity=0.6] (o2b) -- (z3);
%      \draw[opacity=0.6] (o2b) -- (z4);
%      \draw[opacity=0.6] (o2b) -- (z5);

%      \draw[opacity=0.6] (o3b) -- (z1);
%      \draw[opacity=0.6] (o3b) -- (z2);
%      \draw[opacity=0.6] (o3b) -- (z3);
%      \draw[opacity=0.6] (o3b) -- (z4);
%      \draw[opacity=0.6] (o3b) -- (z5);

% %% OUTPUT NODES
%     \draw [black, thick] (11.7,-2.4) to [square left brace ] (11.7,2.4);
%     \node[oup] (o1) at (12,-2) {$x_D$};
%     \node[oup] (o2) at (12,0) {$x_j$};
%     \node[oup] (o3) at (12,2) {$x_1$};
%     \draw[dashed] (o1) to (o2);
%     \draw[dashed] (o2) to (o3);
%     \draw [black, thick] (12.3,-2.4) to [square right brace ] (12.3,2.4);

% %% horizontal links
%      \draw[thick,cadmiumred!40] (o1) -- (o1b);
%      \draw[thick,cadmiumred!40] (o2) -- (o2b);
%      \draw[thick,cadmiumred!40] (o3) -- (o3b);

% \end{scope}
% \end{tikzpicture}
% 	%\caption{}
% \end{figure}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% % SKIP RFM
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}[h]
% 	\centering
% \begin{tikzpicture}
% \begin{scope}[local bounding box=graph]

% %% TEXT
%   \node[text width=3cm, align = center] at (-2,-3) {\Large input};
%   \node[text width=3cm, align = center] at (12,-3) {\Large output};
%   %\node[text width=5cm, align = center] at (0.75,4) {\Large $\mathbb{R}^{D_r\times D} \ni (W_{\rm{in}},b_{\rm{in}})$};
%   %\node[text width=3.5cm, align = center] at (8.35,4) {\Large $W\in \mathbb{R}^{D\times D_r}$};
%   %\node[text width=6cm, align = center] at (5,-6.75) {\Large $z_i = \tanh({W_{\rm{in}}}_{i,j} x_j + {b_{\rm{in}}}_i)$};
%   \node[text width=6cm, align = center] at (5,-6.8) {\Large skip connection};


% %% INPUT NODES
%    \draw [black, thick] (-2.3,-2.4) to [square left brace ] (-2.3,2.4);
%    \node[inp] (i1) at (-2,-2) {$x_D$};
%    \node[inp] (i2) at (-2,0) {$x_j$};
%    \node[inp] (i3) at (-2,2) {$x_1$};
%    \draw[dashed] (i1) to (i2);
%    \draw[dashed] (i2) to (i3);
%    \draw [black, thick] (-1.7,-2.4) to [square right brace ] (-1.7,2.4);

% %% horizontal links
%    \node[inp_b] (i1b) at (1.,-2) {};
%    \node[inp_b] (i2b) at (1.,0) {};
%    \node[inp_b] (i3b) at (1.,2) {};

%    \draw[thick,bleudefrance!40] (i1) -- (i1b);
%    \draw[thick,bleudefrance!40] (i2) -- (i2b);
%    \draw[thick,bleudefrance!40] (i3) -- (i3b);

% %% HIDDEN NODES
%    \filldraw[color=orange!40, fill=orange!40, fill opacity=0.1, rounded corners=1cm](4,-5.75) rectangle (6,5.75);

%    \node[hip] (z1) at (5,-5) {$z_{D_r}$};
%    \node[hip] (z2) at (5,0) {$z_\ell$};
%    \node[hip] (z3) at (5,3) {$z_3$};
%    \node[hip] (z4) at (5,4) {$z_2$};
%    \node[hip] (z5) at (5,5) {$z_1$};
%    \draw[dashed] (z1) to (z2);
%    \draw[dashed] (z2) to (z3);
    
% %% draw lines input --> hidden
%    \draw[opacity=0.6] (i1b) -- (z1);
%    \draw[opacity=0.6] (i1b) -- (z2);
%    \draw[opacity=0.6] (i1b) -- (z3);
%    \draw[opacity=0.6] (i1b) -- (z4);
%    \draw[opacity=0.6] (i1b) -- (z5);
        
%    \draw[opacity=0.6] (i2b) -- (z1);
%    \draw[opacity=0.6] (i2b) -- (z2);
%    \draw[opacity=0.6] (i2b) -- (z3);
%    \draw[opacity=0.6] (i2b) -- (z4);
%    \draw[opacity=0.6] (i2b) -- (z5);

%    \draw[opacity=0.6] (i3b) -- (z1);
%    \draw[opacity=0.6] (i3b) -- (z2);
%    \draw[opacity=0.6] (i3b) -- (z3);
%    \draw[opacity=0.6] (i3b) -- (z4);
%    \draw[opacity=0.6] (i3b) -- (z5);


% %% draw lines hidden --> output 
%    \node[oup_b] (o1b) at (9,-2) {};
%    \node[oup_b] (o2b) at (9,0) {};
%    \node[oup_b] (o3b) at (9,2) {};

%    \draw[opacity=0.6] (o1b) -- (z1);
%    \draw[opacity=0.6] (o1b) -- (z2);
%    \draw[opacity=0.6] (o1b) -- (z3);
%    \draw[opacity=0.6] (o1b) -- (z4);
%    \draw[opacity=0.6] (o1b) -- (z5);
        
%    \draw[opacity=0.6] (o2b) -- (z1);
%    \draw[opacity=0.6] (o2b) -- (z2);
%    \draw[opacity=0.6] (o2b) -- (z3);
%    \draw[opacity=0.6] (o2b) -- (z4);
%    \draw[opacity=0.6] (o2b) -- (z5);

%    \draw[opacity=0.6] (o3b) -- (z1);
%    \draw[opacity=0.6] (o3b) -- (z2);
%    \draw[opacity=0.6] (o3b) -- (z3);
%    \draw[opacity=0.6] (o3b) -- (z4);
%    \draw[opacity=0.6] (o3b) -- (z5);

% %% OUTPUT NODES
%    \draw [black, thick] (11.7,-2.4) to [square left brace ] (11.7,2.4);
%    \node[oup] (o1) at (12,-2) {$x_D$};
%    \node[oup] (o2) at (12,0) {$x_j$};
%    \node[oup] (o3) at (12,2) {$x_1$};
%    \draw[dashed] (o1) to (o2);
%    \draw[dashed] (o2) to (o3);
%    \draw [black, thick] (12.3,-2.4) to [square right brace ] (12.3,2.4);

% %% horizontal links
%    \draw[thick,cadmiumred!40] (o1) -- (o1b);
%    \draw[thick,cadmiumred!40] (o2) -- (o2b);
%    \draw[thick,cadmiumred!40] (o3) -- (o3b);
     
% %% SKIP CONNECTION
%    \coordinate (s0) at (-2,-3.5);
%    \coordinate (s1) at (-2,-6.25);
%    \coordinate (s2) at (12,-6.25);
%    \coordinate (s3) at (12,-3.5);
%    \node[inner sep=0] (sx) at (5,-6.25) {\Large \bf $\oplus$}; 
%    \draw [black,thick] (s0)--(s1);
%    \draw [black,thick] (s1)--(sx);
%    \draw [black,thick] (sx)--(s2);
%    \draw [black,thick,-stealth] (s2)--(s3);

% \end{scope}
% \end{tikzpicture}
% 	%\caption{}
% \end{figure}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% % DEEP SKIP RFM
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \end{document}



==> tikz/local.tex <==
% \documentclass{standalone}
% \usepackage{tikz}
% \usepackage{amsmath, amssymb}
% \usetikzlibrary{arrows,positioning,shapes,decorations.pathreplacing}
% \begin{document}
% \begin{tikzpicture}[node distance=2.5cm]
%     % Define the top rectangles with styles
%     \node (A) [draw, dashed, rectangle, minimum height=1.5cm, minimum width=2cm] {local unit};
%     \node (L) [draw, dashed, rectangle, minimum height=1.5cm, minimum width=2cm, left of=A] {local unit};
%     \node (B) [draw, dashed, rectangle, minimum height=1.5cm, minimum width=2cm, right of=A] {local unit};
%     \node (C) [draw, rectangle, minimum height=1.5cm, minimum width=2cm, right of=B] {local unit};
%     \node (D) [draw, dashed, rectangle, minimum height=1.5cm, minimum width=2cm, right of=C] {local unit};
%     \node (E) [draw, dashed, rectangle, minimum height=1.5cm, minimum width=2cm, right of=D] {local unit};
%     \node (R) [draw, dashed, rectangle, minimum height=1.5cm, minimum width=2cm, right of=E] {local unit};

%     % Define the bottom rectangles
%     \node (L1) [draw, rectangle, minimum height=0.3cm, minimum width=1.5cm, below=0.5cm of L] {};
%     \node (A1) [draw, rectangle, minimum height=0.3cm, minimum width=1.5cm, below=0.5cm of A] {};
%     \node (B1) [draw, rectangle, minimum height=0.3cm, minimum width=1.5cm, below=0.5cm of B] {};
%     \node (C1) [draw, rectangle, minimum height=0.3cm, minimum width=1.5cm, below=0.5cm of C] {};
%     \node (D1) [draw, rectangle, minimum height=0.3cm, minimum width=1.5cm, below=0.5cm of D] {};
%     \node (E1) [draw, rectangle, minimum height=0.3cm, minimum width=1.5cm, below=0.5cm of E] {};
%     \node (R1) [draw, rectangle, minimum height=0.3cm, minimum width=1.5cm, below=0.5cm of R] {};

%     % Define the top smaller rectangles
%     \node (L2) [draw, rectangle, minimum height=0.3cm, minimum width=1.5cm, above=0.5cm of L] {};
%     \node (A2) [draw, rectangle, minimum height=0.3cm, minimum width=1.5cm, above=0.5cm of A] {};
%     \node (B2) [draw, rectangle, minimum height=0.3cm, minimum width=1.5cm, above=0.5cm of B] {};
%     \node (C2) [draw, rectangle, minimum height=0.3cm, minimum width=1.5cm, above=0.5cm of C] {};
%     \node (D2) [draw, rectangle, minimum height=0.3cm, minimum width=1.5cm, above=0.5cm of D] {};
%     \node (E2) [draw, rectangle, minimum height=0.3cm, minimum width=1.5cm, above=0.5cm of E] {};
%     \node (R2) [draw, rectangle, minimum height=0.3cm, minimum width=1.5cm, above=0.5cm of R] {};

%     % Place the circles inside the bottom rectangles
%     \foreach \x in {L1, A1, B1, C1, D1, E1, R1} {
%         \node[circle, draw, fill=blue, inner sep=0pt, minimum size=0.2cm] at ([xshift=-0.5cm] \x.center) {};
%         \node[circle, draw, fill=blue, inner sep=0pt, minimum size=0.2cm] at (\x.center) {};
%         \node[circle, draw, fill=blue, inner sep=0pt, minimum size=0.2cm] at ([xshift=0.5cm] \x.center) {};
%     }

%     % Place the circles inside the top rectangles
%     \foreach \x in {L2, A2, B2, C2, D2, E2, R2} {
%         \node[circle, draw, fill=red, inner sep=0pt, minimum size=0.2cm] at ([xshift=-0.5cm] \x.center) {};
%         \node[circle, draw, fill=red, inner sep=0pt, minimum size=0.2cm] at (\x.center) {};
%         \node[circle, draw, fill=red, inner sep=0pt, minimum size=0.2cm] at ([xshift=0.5cm] \x.center) {};
%     }

%     % Define the paths
%     % \path[->] (A1) edge[bend right=34] node[below] {} (C);
%     \path[->] (A1) edge[bend right=42] node[below] {} (C);
%     \path[->] (B1) edge[bend right=25] node[below] {} (C);
%     \path[->] (D1) edge[bend left=25] node[below] {} (C);
%     % \path[->] (E1) edge[bend left=34] node[below] {} (C);
%     \path[->] (C1) edge[] node[below] {} (C);
%     \path[->] (C) edge[] node[below] {} (C2);
%     \path[->] (E1) edge[bend left=42] node[below] {} (C);
   

%     % Add dashed paths
%     \path[->, dashed] (L) edge[] (L2);
%     \path[->, dashed] (A) edge[] (A2);
%     \path[->, dashed] (B) edge[] (B2);
%     \path[->, dashed] (D) edge[] (D2);
%     \path[->, dashed] (E) edge[] (E2);
%     \path[->, dashed] (R) edge[] (R2);

    
%     % Add the text 
%     \node[below=0.01cm of L1] {$G$};
%     \node[below=0.01cm of A1] {$G$};
%     \node[below=0.01cm of B1] {$G$};
%     \node[below=0.01cm of C1] {$G$};
%     \node[below=0.01cm of D1] {$G$};
%     \node[below=0.01cm of E1] {$G$};
%     \node[below=0.01cm of R1] {$G$};

%     \node[above=0.02cm of L2] {$G$};
%     \node[above=0.02cm of A2] {$G$};
%     \node[above=0.02cm of B2] {$G$};
%     \node[above=0.02cm of C2] {$G$};
%     \node[above=0.02cm of D2] {$G$};
%     \node[above=0.02cm of E2] {$G$};
%     \node[above=0.02cm of R2] {$G$};

%     % \node[above=0.1cm of C2] {state at $t+1$};

%     % Add the bottom underbrace
%     \node (brace start) at ([xshift=-1.3cm, yshift=-0.5cm]L1.south west) {};
%     \node (brace end) at ([xshift=1.3cm, yshift=-0.5cm]R1.south east) {};
%     \draw[decorate,decoration={brace,mirror,amplitude=10pt}] (brace start) -- (brace end) 
%         node[midway,below=10pt] {$N_gG=D$-dimensional state $\mathbf{u}_n$};

%     % Add the top underbrace
%     \node (brace start) at ([xshift=-1.3cm, yshift=0.5cm]L2.north west) {};
%     \node (brace end) at ([xshift=1.3cm, yshift=0.5cm]R2.north east) {};
%     \draw[decorate,decoration={brace,amplitude=10pt}] (brace start) -- (brace end) 
%         node[midway,above=10pt] {estimate of $\mathbf{u}_{n+1}$}; 

%      % Add ellipses
%     \node at ([xshift=-0.5cm]L.west) {\huge $\dots$};
%     \node at ([xshift=0.5cm]R.east) {\huge $\dots$};
% \end{tikzpicture}

% \end{document}


